Learning First-Order Representations for Planning from Black-Box States: New Results

Recently Bonet and Geffner have shown that first-order representations for planning domains can be learned from the structure of the state space without any prior knowledge about the action schemas or domain predicates. For this, the learning problem is formulated as the search for a simplest first-order domain description D that along with information about instances I_i (number of objects and initial state) determine state space graphs G(P_i) that match the observed state graphs G_i where P_i = (D, I_i). The search is cast and solved approximately by means of a SAT solver that is called over a large family of propositional theories that differ just in the parameters encoding the possible number of action schemas and domain predicates, their arities, and the number of objects. In this work, we push the limits of these learners by moving to an answer set programming (ASP) encoding using the CLINGO system. The new encodings are more transparent and concise, extending the range of possible models while facilitating their exploration. We show that the domains introduced by Bonet and Geffner can be solved more efficiently in the new approach, often optimally, and furthermore, that the approach can be easily extended to handle partial information about the state graphs as well as noise that prevents some states from being distinguished.

==> asp_encoding_revised.tex <==

\section{Basic ASP Encoding}

\citeauthor{bonet:ecai2020} \shortcite{bonet:ecai2020} address the learning and verification problems above
as \textbf{SAT problems} using a vector of hyperparameters $\alpha$ to represents the \emph{exact}
number of action schemas and the arity of each one of them, the number of predicate symbols
and the arity of each one of them, the number of different atoms in the schemas,
the total number of unary and binary static predicates, and the number of objects.
Since the true value of these parameters is not known, they use suitable bounds on them,
and generate a propositional theory $T_\alpha(G)$ for each vector of hyperparameters $\alpha$
that complies with these bounds, where $G$ is the input graph (a single input graph is shown
to be enough for learning the representations). Depending on the number of action labels
used in $G$, the number of resulting theories range from 6,390 (Hanoi, 1 label),
to 19,050 (Blockworld and Gripper, 3 labels) and 37,800 (Grid, 4 labels). They
then sample 10\% of these theories, and pass them to a SAT solver. Even with exact
hyperparameters, the \emph{average} time for solving each of these theories remains high,
from 1,400 to 1,800 seconds for Blocks, Hanoi, and Gripper. This is in part because
the SAT theories are large, somewhat complex, and often UNSAT.

Our move from SAT to ASP is motivated to get more compact and transparent encodings
that are easier to understand and explore, and that for this reason, could also
deliver superior performance. Fortunately, this has been achieved, after careful
testing and evaluation. We present the resulting encodings in two parts, first
a basic ASP encoding that is easier to follow and understand, and then the
required optimizations. In these encodings, the learning problems considered by \citeauthor{bonet:ecai2020}
are solved by a handful of calls to the ASP solver \clingo \cite{torsten:asp,torsten:clingo},
as opposed to the thousands of calls required in the original SAT encoding. Moreover, once a preference ordering on solutions is defined,
some of these problems are shown to be solved \emph{optimally}, meaning there is
no simpler representation compatible with the input data.

\subsection{Program}

The ASP code \aspg for learning a first-order instance $P\,{=}\,\tup{D,I}$ from a single input graph $G$
is shown in Figure~\ref{fig:program}. The code can be easily generalized to learn the instances
$P_i\,{=}\,\tup{D,I_i}$ from multiple input graphs $G_i$. The graph $G$ is assumed to be encoded using the
atoms \atom|node(S)| and \atom|tlabel(T,L)| where \atom|S| and \atom|T=(S1,S2)| denote nodes and transitions
in the graph $G$, and \atom|L| denotes the corresponding action label.
The resulting lifted action schemas are encoded via the \atom|prec/3| and \atom|eff/3| atoms (the integer at
the end denotes the arity of the atom), while the factored states
of the nodes \atom|S|, via the \atom|val/2| and \atom|val/3| atoms, the first for static atoms and
the second for dynamic ones. The {main constraints} are at the bottom of the program in Fig.~\ref{fig:program}: transitions \atom|(S1,S2)| are assigned
exactly to one ground action through the atoms \atom|next(A,OO,S1,S2)| where \atom|OO| are the objects that instantiate
the arguments of the action schema \atom|A|. As a result, the value of the ground atoms in the states \atom|S1| and \atom|S2|
has to be compatible with this ground action. In addition, the ground action \atom|A(OO)| has to be applicable in \atom|S1|,
and if it is applicable in a node \atom|S1'|, then there has to be a node \atom|S2'| such that \atom|next(A,OO,S1',S2')| is true.
Also, the sets of literals true in a node (the states associated to nodes) have to be different for different nodes.
The static predicates and atoms refer to those that control the grounding; i.e., they appear in the precondition of
action schemas but do not appear in action effects, so the value of static atoms do not depend on the state
(and hence \atom|val| atoms for static ground atoms do not include an state argument).

The first part of the program (lines 1--\ref{asp:bounds:end}) sets up the bounds on the domain parameters: max number of predicates (5) and static predicates (2),
and max numbers of effects and preconditions per action schema (6). In addition, the arity of actions is bounded by 3, and the
arity of predicates by 2. The number of action schemas is set to the number of action labels, and the number of objects is
fixed to the constant \atom|num\_objects| that is passed to the solver. In our experiments, the solver is instantiated
with values $1,\ldots,10$ for this constant; i.e., for each input graph, the solver is called up to 10 times,
a number that is orders of magnitude smaller than the number of calls in the SAT approach.
%The reason for treating the number of objects in a different way than the other parameters
%is that when the value for the number of objects is left open, the search becomes less effective.

The second part (lines \ref{asp:lifted:begin}--\ref{asp:lifted:end}) sets up
the action schemas and their lifted preconditions and effects, while the
third part (lines \ref{asp:grounding:begin}--\ref{asp:grounding:end}) encodes
the grounding: for a given number of objects, it generates the possible object tuples \atom|OO|
that can instantiate the arguments of action schemas and predicates. % inside such action schemas.
Pairs \atom|(A,OO)| and \atom|(P,OO)| denote ground actions and
ground atoms. Atoms \atom|map(VV,OO1,OO2)| tell that the variable list
\atom|VV| instantiates to \atom|OO2| for the ground instantiation \atom|OO1|
of variables.
%, with the clauses for \atom|map(Pargs,Args,Objs)| encoding that the lifted
% predicate arguments \atom|Pargs| of an an action schema whose arguments have
% been instantiated to \atom|Args|, should be instantiated to \atom|Objs|.
Truth values \atom|V| of ground atoms \atom|(P,OO)| in the state
\atom|S| are encoded with atoms \atom|val((P,OO),S,V)|, with the state
\atom|S| omitted for static predicates.

The last part (lines \ref{asp:last:begin}--\ref{asp:last:end}) encodes the main constraints:
1)~if the ground action \atom|(A,OO)| is assigned to edge \atom|(S1,S2)|, it must be applicable in \atom|S1|,
the values of the ground literals in \atom|S1| and \atom|S2| must be consistent with the action effects, % and non-effects,
and the action labels must coincide,
2)~if the ground action \atom|(A,OO)| is applicable in a node, it must be associated with exactly one of the outgoing edges, and
3)~the sets of true ground literals for different nodes must be different.
The correctness of the encoding can be expressed as follows: %(** need rephrasing and extra conditions, and proof, although not in submission. Define $ASP(G)$. ***)

\begin{theorem}
  Let $G$ be an input graph encoded with the \atom|node/2| and \atom|tlabel/2| atoms.
  Then $M$ is an answer set of the program \aspg iff
  there is a planning instance $P\,{=}\,\pair{D,I}$ that accounts for $G$
  and is compatible with the given bounds; $D$ and $I$ can be read off from such an $M$.
\end{theorem}

\begin{figure*}
  \begin{Verbatim}[gobble=4,frame=single,numbers=left,fontsize=\small,codes={\catcode`$=3}]
    \textcolor{blue}{% Constants}
    #const max_predicates=5.
    #const max_static_predicates=2.
    #const max_effects=6.           % for each action
    #const max_precs=6.             % for each action

    \textcolor{blue}{% Actions, predicates, static predicates and objects}
    action(L) :- tlabel(T,L).
    \{ a_arity(A,1..3) \} = 1 :- action(A).  \textcolor{red}{%%% WHAT ABOUT NULLARY ACTIONS?}
    pred(1..max_predicates).
    \{ p_arity(P,1..2) \} = 1 :- pred(P).
    p_static(max_predicates-max_static_predicates+1..max_predicates).
    object(1..num_objects).\label{asp:bounds:end}

    \textcolor{blue}{% Tuples of variables for lifted effects and preconditions}\label{asp:lifted:begin}
    argtuple((V1,  )) :- V1=1..3.
    argtuple((V1,V2)) :- V1=1..3, V2=1..3.

    \textcolor{blue}{% Generate lifted preconditions and effects (at least 1) of action schemas}
!% at least one effect? (yes if there are no 0-length loops) excludes static predicates
      \{ prec(A,(P,T),0..1) : pred(P), argtuple(T)                  \}   max_precs :- action(A).
    1 \{  eff(A,(P,T),0..1) : pred(P), argtuple(T), not p_static(P) \} max_effects :- action(A).

    \textcolor{blue}{% Check that variables mentioned in precs and effects are action arguments}
    :-  eff(A,(_,(V, )),_), a_arity(A,ARITY), ARITY < V.
    :-  eff(A,(_,(V,_)),_), a_arity(A,ARITY), ARITY < V.
    :-  eff(A,(_,(_,V)),_), a_arity(A,ARITY), ARITY < V.
    :- prec(A,(_,(V, )),_), a_arity(A,ARITY), ARITY < V.
    :- prec(A,(_,(V,_)),_), a_arity(A,ARITY), ARITY < V.
    :- prec(A,(_,(_,V)),_), a_arity(A,ARITY), ARITY < V.

    \textcolor{blue}{% Tuples of objects for grounding the action schemas and atoms}
    objtuple((O1,     ),1) :- object(O1).
    objtuple((O1,O2   ),2) :- object(O1), object(O2).
    objtuple((O1,O2,O3),3) :- object(O1), object(O2), object(O3).\label{asp:lifted:end}

    \textcolor{blue}{% Possible values of ground atoms in the states associated to nodes}\label{asp:grounding:begin}
    \{ val((P,OO),  0..1) \} = 1 :- pred(P),     p_static(P), objtuple(OO,1..2).
    \{ val((P,OO),S,0..1) \} = 1 :- pred(P), not p_static(P), objtuple(OO,1..2), node(S).

    \textcolor{blue}{% Map selects grounding of lifted atoms in schema from grounding of action arguments}
    map( (1,),     (O1,),  (O1,)) :-      objtuple((O1,),1).
    map( (1,),   (O1,O2),  (O1,)) :-    objtuple((O1,O2),1).
    ...
    map((1,1),     (O1,),(O1,O1)) :-      objtuple((O1,),1).
    map((1,1),   (O1,O2),(O1,O1)) :-    objtuple((O1,O2),2).
!map((1,2),   (O1,O2),(O1,O2)) :-    objtuple((O1,O2),2).
!map((2,1),   (O1,O2),(O2,O1)) :-    objtuple((O1,O2),2).
!map((2,2),   (O1,O2),(O2,O2)) :-    objtuple((O1,O2),2).
!map((1,1),(O1,O2,O3),(O1,O1)) :- objtuple((O1,O2,O3),3).
!map((1,2),(O1,O2,O3),(O1,O2)) :- objtuple((O1,O2,O3),3).
!map((1,3),(O1,O2,O3),(O1,O3)) :- objtuple((O1,O2,O3),3).
!map((2,1),(O1,O2,O3),(O2,O1)) :- objtuple((O1,O2,O3),3).
!map((2,2),(O1,O2,O3),(O2,O2)) :- objtuple((O1,O2,O3),3).
!map((2,3),(O1,O2,O3),(O2,O3)) :- objtuple((O1,O2,O3),3).
!map((3,1),(O1,O2,O3),(O3,O1)) :- objtuple((O1,O2,O3),3).
!map((3,2),(O1,O2,O3),(O3,O2)) :- objtuple((O1,O2,O3),3).
!map((3,3),(O1,O2,O3),(O3,O3)) :- objtuple((O1,O2,O3),3).
!map((1,1),(O1,O2,O3),(O1,O1)) :- objtuple((O1,O2,O3),3).
!map((1,2),(O1,O2,O3),(O1,O2)) :- objtuple((O1,O2,O3),3).
!map((1,3),(O1,O2,O3),(O1,O3)) :- objtuple((O1,O2,O3),3).
!map((2,1),(O1,O2,O3),(O2,O1)) :- objtuple((O1,O2,O3),3).
!map((2,2),(O1,O2,O3),(O2,O2)) :- objtuple((O1,O2,O3),3).
!map((2,3),(O1,O2,O3),(O2,O3)) :- objtuple((O1,O2,O3),3).
    ...
!map((3,1),(O1,O2,O3),(O3,O1)) :- objtuple((O1,O2,O3),3).
    map((3,2),(O1,O2,O3),(O3,O2)) :- objtuple((O1,O2,O3),3).
    map((3,3),(O1,O2,O3),(O3,O3)) :- objtuple((O1,O2,O3),3).

    \textcolor{blue}{% Check preconditions: ground action A(OO1) is applicable in node S}
    appl(A,OO1,S) :- action(A), a_arity(A,ARITY), objtuple(OO1,ARITY), node(S),
                     val((P,OO2),  V) : prec(A,(P,T),V), map(T,OO1,OO2),     p_static(P);
                     val((P,OO2),S,V) : prec(A,(P,T),V), map(T,OO1,OO2), not p_static(P).

    \textcolor{blue}{% If ground action A(OO) applicable in S1, assigned to some edge (S1,S2) with same label}
    \{ next(A,OO,S1,S2) : tlabel((S1,S2),A) \} = 1 :- appl(A,OO,S1).\label{asp:grounding:end}

    \textcolor{blue}{% Every edge is assigned to a ground action with the same label}\label{asp:last:begin}
    :- tlabel((S1,S2),A), \{ next(A,OO,S1,S2) \} $\neq$ 1.

    \textcolor{blue}{% Effects and inertia}
!% if (S1,A,S2) with O1 in V1 and O2 in V2,% then the effects must hold in S2
    :- eff(A,(P,T),V), next(A,OO1,S1,S2), map(T,OO1,OO2), val((P,OO2),S2,1-V).
    :- tlabel((S1,S2),_), val(K,S1,V), val(K,S2,1-V), not caused(S1,S2,K).
    caused(S1,S2,(P,OO2)) :- eff(A,(P,T),V), next(A,OO1,S1,S2), map(T,OO1,OO2).
!%
!% Another option for inertia with a single rule:
!% if A(OO1) is applicable in S1 and is connected to S2,
!% if P(OO2) changes its value
!% then there must be some effect accounting for the change
!% :- next(A,OO1,S1,S2), val((P,OO2),S1,V), val((P,OO2),S2,1-V),
!%    not eff(A,(P,T),1-V) : map(T,OO1,OO2).

    \textcolor{blue}{% Different nodes are different states}
    :- node(S1), node(S2), S1 < S2, val((P,T),S2,V) : val((P,T),S1,V).\label{asp:last:end}
!%
!% Display
!#show eff/3.
!#show prec/3.
!#show labelname/2.
!#show val(K,S) : val(K,S,1).
!#show val(K  ) : val(K,  1).
!#show object/1.
  \end{Verbatim}
  \vskip -1em
  \caption{Base code of ASP program \aspg for learning a first-order planning instance $P\,{=}\,\tup{D,I}$
    from a single input graph $G$. The graph $G$ is assumed to be encoded with atoms \atom|node(S)| and
    \atom|tlabel(T,L)| %$node(S)$ and $tlabel(T,L)$   atoms
    where \atom|T=(S1,S2)| stands for the transitions in the graph and \atom|L| for the corresponding
    action label. See text for explanations. %** Problem compiling ``atoms'' **
  }
  \label{fig:program}
\end{figure*}


